Probabilistic Modelling of the Impact on Bus Punctuality of a Speed Limit Proposal in Edinburgh (Extended Version)

We propose a data-driven methodology for evaluating the impact of the introduction of a speed limit on the punctuality of bus services. In particular, we use high-frequency Automatic Vehicle Location data to parameterise a model that represents the movement of a bus along predefined patches of the route. We fit the probability distributions of the time spent in each patch to two classes of probability distributions: hyper-Erlang distributions, for which we use the tool HyperStar, and a variation of the three-parameter gamma distributions recommended by the Traffic Engineering Handbook. In both cases we obtain models that can be expressed using the framework of Probabilistic Timed Automata, allowing us to evaluate bus punctuality using the model checking tool UPPAAL. We conduct a case study involving a proposed speed limit in Edinburgh. This is an extended version of a paper presented at ValueTools 2015.

==> analysis.tex <==
\subsection{UPPAAL Model Construction}


We build our model in Uppaal using the hyper-Erlang parameters for each patch. Each of our models in Uppaal represents a single direction of travel from the moment a bus leaves its starting stop and then enters its final stop as shown in Figure \ref{fig:patchtimeswithends1} and thus excludes the time distributions for both terminating point patches. This was intentional as there is no real need to explicitly model these times as we cannot easily reference it to a time table schedule. As such, we use a minimum of two models to represent a route which can be extended even further to include distinct models for different times of day e.g., for the Airlink (route 100) we can build a model for the morning rush hour (07:00 to 09:00) heading from the Airport to Waverley Bridge. 

As mentioned in our \textit{Background} (Section 2), Uppaal is a powerful model checking tool that allows verification and reachability tests in timed automata systems. As Uppaal has recently incorporated Probabilistic Timed Automata and Statistical Model Checking, we are now able to fully represent the behavior of Phase-Type distributions such as hyper-Erlangs in Uppaal. This provides the ability to check probabilities of our system reaching its end state in a certain time window. 

Uppaal allows us to represent out Erlang phases ($k$) as states, connected by edges, which transition according to a specified rate exponential ($\lambda$). Additionally, it allows the representation of the probabilistic choice ($\alpha_{m}$) between Erlang branches (see Figure \ref{fig:Uppaaldemo1}).



Uppaal stores the structure of each model as a Extensible Markup Language (\textit{XML}) file format. Upon examining the structure of this file, we created a function in \textit{R} to convert our table of hyper-Erlang parameters into an XML that accurately represented our model. We do not the describe algorithm we developed for converting our table of hyper-Erlang parameters to Uppaal's \textit{XML} file, as it is long and quite complicated, however we will describe the basic principles used to construct it. The \textit{XML} contains information regarding the positions of all nodes and whether they contain a rate of an exponential distribution. In addition, it stores all transitions between nodes, indicating if there were any probabilistic transitions between nodes. We should note that Uppaal does not allow non-interger values for probabilistic transitions. Consequently, we had to convert all $\alpha$ values to ratios e.g. if $\alpha_{1} = 0.4938$ and $\alpha_{2} = 0.5062$, Uppaal requires we set the probabilistic transition ratio as 2469:2531 which was found by converting the decimal to a fraction and using the numerators for this ratio. We now show in Figure \ref{fig:uppaalformat}, an illustration of major segments that make up the Uppaal \textit{XML}, followed by the Uppaal graphic editor view of its representation (color coded).


%\begin{figure}[!htbp]
	%\centerline{\includegraphics[width=0.46\textwidth]{figures/uppaalformat.png}}
    %\caption{Description of Uppaal's XML format}
    %\label{fig:uppaalformat}
%\end{figure}
%
%\begin{figure}[!htbp]
	%\centerline{\includegraphics[width=0.46\textwidth]{figures/uppaalmodel.png}}
    %\caption{Description of Uppaal's XML format}
    %\label{fig:uppaalmodel}
%\end{figure}

Our function converts the hyper-Erlang parameters to Uppaal's \textit{XML} file thus providing a fully constructed model. Our Uppaal model can now be used to perform probability queries, thus providing us with the ability to compare the behavior of models with and without speed limits enforced. Queries take the form off \textit{What is the probability of completing this route in less than 36 minutes?}. In Uppaal's querying language, this takes the form of \textbf{\textit{Pr[$<=$2160] ($<>$ Process.end)}}, which means what is the probability of reaching the \textit{end} state in less than 2,160 seconds. After a certain number of runs, Uppaal produces an output in the form \textbf{(1354 runs) Pr($<>$ ...) in [0.98646,0.996453] with confidence 0.95.}, which provides us with a so-called confidence interval for the probability estimate of our query.

\subsection{Parameter Fitting Results}

Note that Patch 11 is not included as it is a one-way patch and all measurements were counted as belonging to the other direction.

%
%\begin{table}
	%\centering
		%\begin{tabular}{ccc}
		  %\hline
			%Patch & with & without \\
			%\hline
			%1 & 50 & 60 \\
			%\hline
		%\end{tabular}
%\end{table}

\begin{table}
	\centering
		\begin{tabular}{ccccc}
		  \hline
			 & & \multicolumn{2}{c}{hyper-Erlang} & \\
			Patch & Erlang & 2-branch & 3-branch & Erlang+constant\\
			\hline
			%1 & -112.07 & -97.97 & -97.65 & -105.46 \\
			%2 & -93.72 & -93.29 & -93.29 & -91.40 \\
			%3 & -92.98 & -93.80 & -91 & -92.78 \\
			%4 &  & -380 & -360 & -126.51 \\
			%5 & -400 & -380 & -360 & -92.30 \\
			%6 & -400 & -380 & -360 & -89.00 \\
			%7 & -400 & -380 & -360 & -83.11 \\
			%8 & -400 & -380 & -360 & -110.12 \\
			%9 & -400 & -380 & -360 & -51.25 \\
			%10 & -400 & -380 & -360 & -76.34 \\
			%1 & -330.28 & -334.64 & -327.83 & -329.519461559899 \\
			%2 & -453.17 & -386.69 & -386.69 & -426.587146656834 \\
			%3 & -346.91 & -345.35 & -347.16 & -344.936041745722 \\
			%4 & -376.54 & -369.18 & -370.80 & -370.874986779885 \\
			%5 & -329.78 & -330.80 & -327.23 & -328.275905204163 \\
			%6 & -284.65 & -276.49 & -277.90 & -280.864896561775 \\
			%7 & -356.08 & -354.99 & -356.81 & -352.212808292689 \\
			%8 & -403.78 & -406.27 & -403.75 & -403.420196675078 \\
			%9 & -398.19 & -403.31 & -392.34 & -398.17216958321 \\
			%10 & -427.94 & -427.44 & -424.74 & -427.487724199713 \\
			1 & -330.28 & -327.12 & -325.91 & -329.52 \\
			2 & -453.17 & -386.69 & -379.07 & -426.59 \\
			3 & -346.91 & -345.35 & -347.19 & -344.94 \\
			4 & -376.54 & -369.18 & -369.79 & -370.87 \\
			5 & -329.78 & -330.54 & -327.11 & -328.28 \\
			6 & -284.65 & -276.49 & -277.07 & -280.86 \\
			7 & -356.08 & -354.99 & -353.44 & -352.21 \\
			8 & -403.78 & -405.97 & -403.75 & -403.42 \\
			9 & -398.19 & -403.31 & -392.34 & -398.17 \\
			10 & -427.94 & -427.44 & -424.74 & -427.49 \\
			\hline
		\end{tabular}
		\caption{Total log-likelihoods for each of the distributions fitted to the patch journey times in each of the patches for the Airlink, from Waverley Bridge to the airport. }
\end{table}

\begin{table}
	\centering
		\begin{tabular}{ccccc}
		  \hline
			 & & \multicolumn{2}{c}{hyper-Erlang} & \\
			Patch & Erlang & 2-branch & 3-branch & Erlang+constant\\
			\hline
			1 & 91 & 293 & 1030 & 16 \\
			2 & 2 & 63 & 2096 & 1 \\
			3 & 23 & 152 & 681 & 4 \\
			4 & 12 & 94 & 309 & 2 \\
			5 & 30 & 200 & 586 & 7 \\
			6 & 24 & 204 & 537 & 3 \\
			7 & 22 & 144 & 424 & 3 \\
			8 & 8 & 42 & 241 & 4 \\
			9 & 10 & 52 & 227 & 9 \\
			10 & 18 & 148 & 425 & 6 \\
			\hline
		\end{tabular}
		\caption{Phase counts.}
\end{table}

\begin{table*}[!htbp]
\centering
\small
\begin{tabular}{c c c c c c c c}
  \hline
\textbf{Speed Limit Status }$\rightarrow$ & \textbf{Off} & \textbf{On} & \textbf{Off} & \textbf{On} & \textbf{Off} & \textbf{On} & {} \\ 
\textbf{Patch} & \textbf{$\mu_{1}$} &\textbf{ $\mu_{1}$}  &\textbf{ $\mu_{2}$} &\textbf{$\mu_{2}$} & \textbf{$\mu$} & \textbf{$\mu$} &\textbf{ Percent Change in $\mu$ }\\
  \hline
10 & 214.11 & 268.16 & 262.28 & 226.6 & 241 & 251.73 & +4.45\% \\ 
9 & 160.83 & 221.22 & 215.93 & 158.89 & 189.02 & 190.05 & +0.54\% \\ 
8 & 98.29 & 169.03 & 170 & 109.18 & 135.81 & 141.51 & +4.2\% \\  
   \hline
\end{tabular}
\caption{Hyper-Erlang parameters for patch 8,9 and 10 (Airlink - Waverley to Aiport) branch mean comparisons, where $\mu = \alpha_{1}\mu_{1} + \alpha_{2}\mu_{2}$.} 
\label{table:means}
\end{table*} 

\begin{figure*}[!htbp]
	\centering
	\subfloat[][without the speed limit]{\includegraphics[width=0.46\textwidth]{hyper_off.png}\label{fig:speedoff}}
  \subfloat[][with the speed limit]{\includegraphics[width=0.46\textwidth]{hyper_on.png}\label{fig:speedon}}
	%previous name B9on and b9off
	\caption{Aaa}
\end{figure*}
